LinVT: Empower Your Image-level Large Language Model to Understand Videos

Large Language Models (LLMs) have been widely used in various tasks, motivating us to develop an LLM-based assistant for videos. Instead of training from scratch, we propose a module to transform arbitrary well-trained image-based LLMs into video-LLMs (after being trained on video data). To better adapt image-LLMs for processing videos, we introduce two design principles: linear transformation to preserve the original visual-language alignment and representative information condensation from redundant video content. Guided by these principles, we propose a plug-and-play Linear Video Tokenizer(LinVT), which enables existing image-LLMs to understand videos. We benchmark LinVT with six recent visual LLMs: Aquila, Blip-3, InternVL2, Mipha, Molmo and Qwen2-VL, showcasing the high compatibility of LinVT. LinVT-based LLMs achieve state-of-the-art performance across various video benchmarks, illustrating the effectiveness of LinVT in multi-modal video understanding.

==> sec/tables/ablation_token_alignment_scheme.tex <==
\begin{table*}[t!]
\centering
% \resizebox{\textwidth}{!}{
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}c|cccccccccc}
\hline
 & {MVB} & {MMB-V} & {V-MME} & {LongVB} & {N-QA} & {ES} & {MVD-QA} & {MTT-QA} & {Act-QA} & {TGIF-QA}\\
\hline
 a & 62.5 & 1.22 & 48.4 / 49.2 & 49.7 & 71.1 & 55.9 & 71.2/3.8 & 55.3/3.0 & 47.5/3.1 & 71.1/3.9 \\
 b & 61.3 & 1.19 & 47.7 / 48.1 & 46.9 & 72.2 & 53.2 & 71.3/3.8 & 55.3/3.0 & 47.7/3.2 & 70.8/3.9\\
\hline
\end{tabular*}
% }
\caption{(supp.) Performance on video benchmarks. Higher values are preferred for all metrics. text-condition implementation. We conducted ablation experiments on an image-LLM Mipha-1.6B model to compare visual and text token alignment schemes.}
\label{tab:implement_text}
\end{table*}

==> sec/tables/suppl_ablation_svr_tta.tex <==
\begin{table*}[h!]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{cc|ccccccccccc}
\hline
SVR & TTA & {MVB} & {MMB-V} & {V-MME} & {LongVB} & {N-QA} & {EgoS} & {MVD-QA} & {MTT-QA} & {Act-QA} & {TGIF-QA}\\
\hline
& & 41.6 & 0.55 & 30.5 / 30.1 & 31.0 & 40.7 & 29.8 &  35.4 / 1.8 & 24.1 / 1.2 & 20.3 / 1.6 & 33.2 / 1.5 \\
\checkmark & & 60.3 & 1.12 & 45.7 / 46.1 & 46.2 & 67.1 & 51.4 & 67.5 / 3.4 & 52.7 / 2.7 & 46.2 / 2.9 & 68.9 / 3.6\\
& \checkmark & 58.7 & 1.03 & 45.4 / 45.7 & 44.8 & 65.1 & 50.2 & 64.1 / 3.2 & 50.3 / 2.4 & 41.6 / 2.6 & 66.9 / 3.2\\
\checkmark & \checkmark & \textbf{62.5} & \textbf{1.22} & \textbf{48.4} / \textbf{49.2} & \textbf{49.7} & \textbf{71.1} & \textbf{55.9} & \textbf{71.2} / \textbf{3.8} & \textbf{55.3} / \textbf{3.0} & \textbf{47.5} / \textbf{3.1} & \textbf{71.1} / \textbf{3.9} \\
\hline
\end{tabular}%
}
% \vspace{-1em}
\caption{
Ablation studies on the effectiveness of SVR and TTA. The image-LLM used in this experiment is Mipha-1.6B. We include the result of the baseline without the proposed LinVT modules compared to \cref{tab:sub_modules}.}
\label{tab:suppl_sub_modules}
\end{table*}

==> sec/tables/suppl_video_zeroshot.tex <==
\begin{table*}[h!]
\centering
\renewcommand{\arraystretch}{1.2}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|cccc}
\hline
{Method} & {Size} & MVD-QA & MTT-QA & Act-QA & TGIF-QA \\
\hline
BLIP-3-Video~\cite{ryoo2024xgen} & 4B & {77.7 / 4.2} & {60.0 / 3.6} & {\closeruline{55.7} / \closeruline{3.5}} & {76.5 / \textbf{4.3}} \\
\hline
\rowcolor[HTML]{EFEFEF} 
LinVT-BLIP-$3^*$ & 4B & \closeruline{78.1} / \closeruline{4.3} & \closeruline{60.3} / \closeruline{3.8} & 55.6 / \closeruline{3.5} & \closeruline{76.9} / \textbf{4.3} \\
\rowcolor[HTML]{EFEFEF} 
LinVT-BLIP-3     & 4B & \textbf{79.1} / \textbf{4.4} & \textbf{61.5} / \textbf{3.9} & \textbf{58.9} / \textbf{3.6} & \textbf{78.7} / \textbf{4.3} \\
\hline
\end{tabular}%
}
\vspace{-0.5em}
\caption{
Comparison with BLIP-3-Video~\cite{ryoo2024xgen} on four zero-shot video QA datasets. Particularly, * indicates the model trained on the same data as BLIP-3-Video. The best results are in \textbf{bold} and second best \ul{underlined}.
}
\label{tab:suppl_res_openend}
\end{table*}
